Detecting the Insider Threat with Long Short Term Memory (LSTM) Neural Networks

Information systems enable many organizational processes in every industry. The efficiencies and effectiveness in the use of information technologies create an unintended byproduct: misuse by existing users or somebody impersonating them - an insider threat. Detecting the insider threat may be possible if thorough analysis of electronic logs, capturing user behaviors, takes place. However, logs are usually very large and unstructured, posing significant challenges for organizations. In this study, we use deep learning, and most specifically Long Short Term Memory (LSTM) recurrent networks for enabling the detection. We demonstrate through a very large, anonymized dataset how LSTM uses the sequenced nature of the data for reducing the search space and making the work of a security analyst more effective.

==> 2.RelatedWork.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Related Work %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Guides:
% - Organize the relevant and recent papers in the corresponding literature into different
%   topics covered by the paper.
% - For each topic discuss the similarity, novelty, or contrast of the paper’s approach.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\vspace{-3mm}
%


Add Related Work here \cite{walker05} and  \cite{integ3} .

==> 7.Conclusion.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CONCLUSION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GUIDES
% - Provide a summary of the paper using the technical terms you used in the paper.
% - Elaborate on important arguments that were derived from the discussions in the paper.
% - Discuss your Future work related to this approach. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\vspace{-3mm}
%
Add your Conclusion here. 
